F3S: Free Flow Fever Screening

Identification of people with elevated body temperature can reduce or dramatically slow down the spread of infectious diseases like COVID-19. We present a novel fever-screening system, F3S, that uses edge machine learning techniques to accurately measure core body temperatures of multiple individuals in a free-flow setting. F3S performs real-time sensor fusion of visual camera with thermal camera data streams to detect elevated body temperature, and it has several unique features: (a) visual and thermal streams represent very different modalities, and we dynamically associate semantically-equivalent regions across visual and thermal frames by using a new, dynamic alignment technique that analyzes content and context in real-time, (b) we track people through occlusions, identify the eye (inner canthus), forehead, face and head regions where possible, and provide an accurate temperature reading by using a prioritized refinement algorithm, and (c) we robustly detect elevated body temperature even in the presence of personal protective equipment like masks, or sunglasses or hats, all of which can be affected by hot weather and lead to spurious temperature readings. F3S has been deployed at over a dozen large commercial establishments, providing contact-less, free-flow, real-time fever screening for thousands of employees and customers in indoors and outdoor settings.

==> files/ref.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{cdc}
\BIBentryALTinterwordspacing
CDC, ``Coronavirus ({COVID}-19),'' 2020. [Online]. Available:
  \url{https://www.cdc.gov/coronavirus/2019-ncov/index.html}
\BIBentrySTDinterwordspacing

\bibitem{ISO/TR13154:2017}
\BIBentryALTinterwordspacing
I.~13154:2017, ``Medical electrical equipment — deployment, implementation
  and operational guidelines for identifying febrile humans using a screening
  thermograph,'' 2017. [Online]. Available:
  \url{https://www.iso.org/standard/69347.html}
\BIBentrySTDinterwordspacing

\bibitem{contactless-vital-signs-2020}
T.~Negishi, S.~Abe, T.~Matsui, H.~Liu, M.~Kurosawa, T.~Kirimoto, and G.~Sun,
  ``Contactless vital signs measurement system using rgb-thermal image sensors
  and its clinical screening test on patients with seasonal influenza,''
  \emph{Sensors}, vol.~20, no.~8, Apr 2020.

\bibitem{applications-irt-2017}
G.~Sun, T.~Matsui, T.~Kirimoto, Y.~Yao, and S.~Abe, \emph{Applications of
  Infrared Thermography for Noncontact and Noninvasive Mass Screening of
  Febrile International Travelers at Airport Quarantine Stations}.\hskip 1em
  plus 0.5em minus 0.4em\relax Springer, 2017.

\bibitem{infrared-thermal-detection-comparisons-2015}
M.~Tay, Y.~Low, X.~Zhao, A.~Cook, and V.~Lee, ``Comparison of infrared thermal
  detection systems for mass fever screening in a tropical healthcare
  setting,'' \emph{Public health}, vol. 129, 08 2015.

\bibitem{stable-contactles-sensing-with-face-2018}
T.~{Negishi}, G.~{Sun}, H.~{Liu}, S.~{Sato}, T.~{Matsui}, and T.~{Kirimoto},
  ``Stable contactless sensing of vital signs using rgb-thermal image fusion
  system with facial tracking for infection screening,'' in \emph{2018 40th
  Annual International Conference of the {IEEE} Engineering in Medicine and
  Biology Society (EMBC)}, 2018.

\bibitem{remote-sensing-CMOS-2017}
G.~Sun, Y.~Nakayama, S.~Dagdanpurev, S.~Abe, H.~Nishimura, T.~Kirimoto, and
  T.~Matsui, ``Remote sensing of multiple vital signs using a cmos
  camera-equipped infrared thermography system and its clinical application in
  rapidly screening patients with suspected infectious diseases,''
  \emph{International Journal of Infectious Diseases}, vol.~55, 01 2017.

\bibitem{multiple-vital-sign-comparisons-2016}
Y.~{Yao}, G.~{Sun}, T.~{Matsui}, Y.~{Hakozaki}, S.~{van Waasen}, and
  M.~{Schiek}, ``Multiple vital-sign-based infection screening outperforms
  thermography independent of the classification algorithm,'' \emph{{IEEE}
  Transactions on Biomedical Engineering}, vol.~63, no.~5, 05 2016.

\bibitem{ici-temperature-screening}
\BIBentryALTinterwordspacing
``Elevated body temperature screening solutions.'' [Online]. Available:
  \url{https://infraredcameras.com/temperature-screening/}
\BIBentrySTDinterwordspacing

\bibitem{lamasatech}
\BIBentryALTinterwordspacing
``{T}emperature {S}creening {K}iosks with {V}isitor and {E}mployee {S}ign-in.''
  [Online]. Available:
  \url{https://www.lamasatech.com/products/interactive-kiosks/body-temperature-kiosk/}
\BIBentrySTDinterwordspacing

\bibitem{ignatiuz}
\BIBentryALTinterwordspacing
``{DA}i{ZO} {COVID} 19 {B}ody {T}emperature {S}creening {K}iosk.'' [Online].
  Available:
  \url{https://www.ignatiuz.com/products/body-temperature-screening-kiosk/}
\BIBentrySTDinterwordspacing

\bibitem{kriosk}
\BIBentryALTinterwordspacing
``Make {W}orkplace {S}afer {W}ith {O}ur {A}ccess {A}nd {T}emperature
  {S}creening {K}iosks.'' [Online]. Available: \url{https://kriosk.com/}
\BIBentrySTDinterwordspacing

\bibitem{fisherstech}
\BIBentryALTinterwordspacing
``{TEMPERATURE KIOSKS}.'' [Online]. Available:
  \url{https://www.fisherstech.com/temperature-kiosks/}
\BIBentrySTDinterwordspacing

\bibitem{diversified}
\BIBentryALTinterwordspacing
``Vital{S}ign {B}ody {T}emperature {C}heck {K}iosk.'' [Online]. Available:
  \url{https://diversifiedus.com/solutions/products/vitalsign-body-temperature-check-kiosk/}
\BIBentrySTDinterwordspacing

\bibitem{body-tempature-crowd-2018}
H.~F. {Haghmohammadi}, D.~S. {Necsulescu}, and M.~{Vahidi}, ``Remote
  measurement of body temperature for an indoor moving crowd,'' in \emph{2018
  {IEEE} Intl. Conf. on Automation, Quality and Testing, Robotics}, 2018.

\bibitem{mobile-platform-2017}
A.~{Somboonkaew}, P.~{Prempree}, S.~{Vuttivong}, J.~{Wetcharungsri},
  S.~{Porntheeraphat}, S.~{Chanhorm}, P.~{Pongsoon}, R.~{Amarit},
  Y.~{Intaravanne}, K.~{Chaitavon}, and S.~{Sumriddetchkajorn},
  ``Mobile-platform for automatic fever screening system based on infrared
  forehead temperature,'' in \emph{2017 Opto-Electronics and Communications
  Conference (OECC) and Photonics Global Conference (PGC)}, 2017.

\bibitem{jangblad2018object}
M.~Jangblad, ``Object detection in infrared images using deep convolutional
  neural networks,'' 2018.

\bibitem{neoface}
\BIBentryALTinterwordspacing
``Face {R}ecognition.'' [Online]. Available:
  \url{https://www.nec.com/en/global/solutions/biometrics/face/index.html}
\BIBentrySTDinterwordspacing

\bibitem{rublee2011orb}
E.~Rublee, V.~Rabaud, K.~Konolige, and G.~Bradski, ``Orb: An efficient
  alternative to sift or surf,'' in \emph{2011 International conference on
  computer vision}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2011.

\bibitem{szeliski2010computer}
R.~Szeliski, \emph{Computer vision: algorithms and applications}.\hskip 1em
  plus 0.5em minus 0.4em\relax Springer Science \& Business Media, 2010.

\bibitem{kingma2014adam}
D.~P. Kingma and J.~Ba, ``Adam: A method for stochastic optimization,'' 2014.

\bibitem{mobotix}
\BIBentryALTinterwordspacing
Mobotix, ``M16 {T}hermal {TR},'' 2020. [Online]. Available:
  \url{https://www.mobotix.com/en/products/thermographic-cameras/m16-thermal-tr}
\BIBentrySTDinterwordspacing

\bibitem{ici-fixed-thermal}
\BIBentryALTinterwordspacing
``F{M} 640 {P}lus {P} {S}eries {IR} {C}amera.'' [Online]. Available:
  \url{https://infraredcameras.com/product/fm-640-plus-p-series-ir-camera/}
\BIBentrySTDinterwordspacing

\bibitem{seek-thermal}
\BIBentryALTinterwordspacing
``Seek {T}hermal.'' [Online]. Available: \url{https://www.thermal.com/}
\BIBentrySTDinterwordspacing

\bibitem{intel-realsense}
\BIBentryALTinterwordspacing
``Intel {R}ealsense cameras.'' [Online]. Available:
  \url{https://www.intelrealsense.com/}
\BIBentrySTDinterwordspacing

\end{thebibliography}

